Surgical task-space optimisation of the CYCLOPS robotic system

The CYCLOPS is a cable-driven parallel mechanism used for minimally invasive applications, with the ability to be customised to different surgical needs; allowing it to be made procedure- and patient-specific. For adequate optimisation, however, appropriate data on clinical constraints and task-space is required. Whereas the former can be provided through preoperative planning and imaging, the latter remains a problem, primarily for highly dexterous MIS systems. The current work focuses on the development of a task-space optimisation method for the CYCLOPS system and the development of a data collection method in a simulation environment for minimally invasive task-spaces. The same data collection method can be used for the development of other minimally invasive platforms. A case-study is used to illustrate the developed method for Endoscopic Submucosal Dissection (ESD). This paper shows that using this method, the system can be succesfully optimised for this application.

==> body/OptimizationAlgorithm.tex <==
The system workspace can be optimised to a specific taskspace by changing the size and shape of the overtube, tendon attachment and feeding points. \\

[TODO: add bit more about objective function, general way]

It is easy to see that the objective function defined is not continuous as the task-space constraint and dexterous workspace calculation involved the testing of discrete points. This favored the use of derivative free direct search methods.

A hybrid particle swarm pattern search algorithm \cite{vaz2009pswarm} was used to perform the optimization. In addition, elements of two other optimization methods, simulated annealing and particle filter optimization, were incorporated to the algorithm.

Simulated annealing in global optimization involves using probability to accept or reject a new position in the search space. When incorporated to the algorithm, a probabilistic method was used to reject the current position of particle in the particle swarm and to resample it from the entire search space. This improved exploration of the parameter space.

Particle filter optimization \cite{ji2008particle} was used at the end of the main algorithm. While particle filters are known to be less effective for high dimensional problems as there are insufficient particles present to fully represent the distribution \cite{gustafsson2010particle}, it was noted that the particle swarm pattern search step had caused a proportion of the particles to move towards areas which are more likely to be the global optimum. Resampling a new set of particles to these areas can help with exploration of these areas and provide a better result.



\subsubsection{Algorithm Implementation}


The final algorithm is outlined as follows

\begin{enumerate}
\item Initialize particle swarm and evaluate objective function for each particle.
\item Begin particle swarm pattern search iterations until stopping criteria is achieved.
\begin{enumerate}
\item Update velocities and positions of particles and evaluate objective function values.
\item If no better position is found, perform pattern search poll step as described in \cite{bogani2009generalized}.
\item Perform simulated annealing based resampling as mentioned above.
\end{enumerate}
\item Initialize new particle swarm where the particles are sampled from previous swarm based on their objective function values.
\item Begin PFO iterations until stopping criteria is achieved.
\begin{enumerate}
\item Update velocities and positions of particles and evaluate objective function values. Update particle weights.
\item Resample particle based on weights to avoid degeneracy problem \cite{gustafsson2010particle}.
\end{enumerate}
\end{enumerate}




==> body/non-opt-cyclops.tex <==
The non-optimized CYCLOPS configuration is based on previous experiences with the system, and can be summarized as a couple rules of thumb. To some extent this already can be seen as an optimisation process, though, the simplicity limits it only to straightforward cases. The rules of thumb are as follows, and figure XX is used to clarify these:\\
- tendons are placed in a 120 degree configuration from each other\\
- largest distance in the x-axis of the task-space determines the difference between length a and b\\
- the ratio between a and c determines the ability to exert large forces on the end-effector. \\

==> body/opt-parameters.tex <==
For adequate comparison between the non-optimised and optimised system, the same parameters are chosen during simulation. These are summarized in table XX. [...MORE..]


==> body/optimisedESD.tex <==

The optimization algorithm was constructed based on a 6-tendon CYCLOPS with a cylindrical scaffold.

\subsubsection{Design Vector}

\begin{figure}
	\centering
	\includegraphics[width=3.5in]{./graphics/PAPER_optimisation-02.jpg}
	\caption{Frame used for optical tracking}
	\label{fig_REALSYSTEM}
\end{figure}

In the optimization algorithm, the following parameters are optimized.
\begin{itemize}
\item Cross-sectional angle for each tendon
\item Attachment point for each tendon
\item Feeding point for front three tendons 
\item Feeding point for back three tendons 
\item Length of the tool
\item Curvature angles and curve position if a curved tool is considered
\end{itemize}

The cross-sectional angle of the tendon refers to the angle which the $yz$-component of the tendon makes with the $y$-axis. The $y$ and $z$ components of the points can be then obtained using trigonometry. If additional tendons were required, 3 parameters per additional tendon would be added to the design vector. They correspond to the cross sectional angle, the attachment point and the feeding point of each additional vector.

The size of the design vector is thus given by $15 + 3(n-6) + 3c$, where n is the number of tendons, and $c \in \{ 0, 1 \}$ depending whether a curvature in the tool is required. 

\subsubsection{Objective Function}
The purpose of the optimization was to generate a CYCLOPS configuration that is superior to the standard configuration. This requires the objective function to return a suitable measure that can be optimized. In this study, the dexterous workspace as defined in \cite{hay2005optimization} was chosen. Additionally, the objective function has to account for the following constraints

% This is for defining your own numbering system without having to import the enumerate package.
\newenvironment{renum}
  {\begin{enumerate}\renewcommand\labelenumi{\roman{enumi}.}}
  {\end{enumerate}}
\begin{renum}
\item Tendons must not cross each other. Considering the attachment points, $\vec{a}$ and feeding points, $\vec{B}$. It must follow that:

\begin{equation}
a_x^i > a_x^j \Rightarrow B_x^i > B_x^j
\end{equation}
\item A configuration where the $x$-distance between the feeding points is smaller than that of the the attachment points is not allowed. As this configuration causes complications in the control of the CYCLOPS.
\item The configuration should be able to able to reach all points in the task-space given.
\end{renum}

The objective function incorporates these constraints and the chosen measure by returning values at different ranges depending on how well the input configuration satisfies the various constraints. Fig.~\ref{fig:objfunction} shows an outline of how this is done. \cite{bryson2016optimal} employs a similar method where the objective function returns a weighted sum of the condition and measure, with the condition having a much larger weight to ensure that it is fulfilled.

\begin{figure}[htpb]
\centering
\includegraphics[width = 1\hsize]{./graphics/objfunc}
\caption{Flowchart of Objective Function}
\label{fig:objfunction} 
\end{figure}

Note that when the dexterous workspace is returned, it's value is made to be negative. The impossible value is also chosen to be greater than 1.

